A Converting Autoencoder Toward Low-latency and Energy-efficient DNN Inference at the Edge

Reducing inference time and energy usage while maintaining prediction accuracy has become a significant concern for deep neural networks (DNN) inference on resource-constrained edge devices. To address this problem, we propose a novel approach based on "converting" autoencoder and lightweight DNNs. This improves upon recent work such as early-exiting framework and DNN partitioning. Early-exiting frameworks spend different amounts of computation power for different input data depending upon their complexity. However, they can be inefficient in real-world scenarios that deal with many hard image samples. On the other hand, DNN partitioning algorithms that utilize the computation power of both the cloud and edge devices can be affected by network delays and intermittent connections between the cloud and the edge. We present CBNet, a low-latency and energy-efficient DNN inference framework tailored for edge devices. It utilizes a "converting" autoencoder to efficiently transform hard images into easy ones, which are subsequently processed by a lightweight DNN for inference. To the best of our knowledge, such autoencoder has not been proposed earlier. Our experimental results using three popular image-classification datasets on a Raspberry Pi 4, a Google Cloud instance, and an instance with Nvidia Tesla K80 GPU show that CBNet achieves up to 4.8x speedup in inference latency and 79% reduction in energy usage compared to competing techniques while maintaining similar or higher accuracy.

==> ML.tex <==
CNN tutorial

%https://medium.com/@RaghavPrabhu/understanding-of-convolutional-neural-network-cnn-deep-learning-99760835f148#:~:text=Stride%20is%20the%20number%20of,with%20a%20stride%20of%202.

%https://machinelearningmastery.com/convolutional-layers-for-deep-learning-neural-networks/

%https://towardsdatascience.com/10-minutes-to-building-a-cnn-binary-image-classifier-in-tensorflow-4e216b2034aa


==> RelatedWork_old.tex <==
\section{related work}
  
There have been a lot of works focusing on solving the problem: Design deep neural network with energy-efficient implementation as well as maintaining the same inference accuracy. Multi-exit architectures that the neural network conditionally with auxiliary classifiers allowing the processing of a test example to terminate earlier depending on the hardness of the input can reduce the inference time and energy consumption without bringing additional accuracy loss.\\
Panda et al proposed Conditional Deep Learning (CDL) where the convolutional layer features are used to identify the variability in the difficulty of input instances and conditionally activate the deeper layers of the network. They achieved this by cascading a linear network of output neurons for each convolutional layer and monitoring the output of the linear network to decide whether classification can be terminated at the current stage or not. The proposed methodology thus enables the network to dynamically adjust the computational effort depending upon the difficulty of the input data while maintaining competitive classification accuracy \cite{panda2016conditional}. Jayakodi et al proposed a principled optimization algorithm to automatically configure C2F Nets for a specified trade-off between accuracy and energy consumption for inference. The key idea is to select a classifier on-the-fly whose complexity is proportional to the hardness of the input example: simple classifiers for easy inputs and complex classifiers for hard inputs \cite{Jayakodi_2018}.
Phuong proposed a new training procedure for multi-exit architectures based on the principle of knowledge distillation. The method encourages early exits to mimic later, more accurate exits, by matching their probability outputs. The method is particularly beneficial when training data is limited and also allows a straight-forward extension to semi-supervised learning, i.e. make use also of unlabeled data at training time. Moreover, it takes only a few lines to implement and imposes almost no computational overhead at training time, and none at all at test time \cite{Phuong2019DistillationBasedTF}.
Park propose Branch-pruned Conditional Neural Network (BPNet) and its methodology in which the time-accuracy tradeoff for the conditional neural network can be found systematically. We applied BPNet to SqueezeNet, ResNet-20, and VGG-16 with CIFAR-10 and 100. BPNet achieves up to 3.15× of speedup without any accuracy drop compared to the base networks\cite{Park-DAC2020}.
Duggal et al propose the EarLy-exiting Framework(ELF) to incorporate this notion of hardness into the learning process. During training, ELF learns to early-exit easy examples through auxiliary branches attached to a backbone network. This offers a dual benefit-(1) the neural network increasingly focuses on hard examples, since they contribute more to the overall network loss; and (2) it frees up additional model capacity to distinguish difficult examples.\cite{duggal2020elf}

In recent times running machine learning algorithm like DNN on resouce constrained edge device has gained significant attention.But, running DNN on this end devices has an overhead of high computation and energy consumption. E. In \cite{li2018edge}, authors addressed this problem and  proposed a new Edgent that adaptively partitions the DNN computation between edge device and accelerate DNN inference through early exit to reduce compuation latency\cite{li2018edge}. DNN partitioning has been explored vigorously recently to minimize energy consumption and latency both for Training and Inferencing.In another work, Yiping et al designed Neurosurgeon, a lightweight scheduler to automatically partition DNN computation between mobile devices and datacenters at the granularity of neural network layers. Their proposed framework adapts to various DNN architectures, hardware platforms, wireless networks, and server load levels, intelligently partitioning computation for best latency or best mobile energy\cite{Kang2017NeurosurgeonCI}. In \cite{9546452} authors proposed a serverless based model serving system named Gillis that automatically partitions a large
model across multiple serverless functions for faster inference and
reduced memory footprint per function. Another containerized partition-based
runtime adaptive convolutional neural network (CNN) acceleration framework for Internet of Things (IoT) environments was stated in \cite{234801}.

For our experiment, we used a power consumption model\cite{Kaup2014PowerPi} for the Raspberry Pi which is used as a substitute to conventional home gateways to derive the impact of typical hardware components on the energy consumption. In their work, different power states are measured and a power model was formulated. The power model can estimate the power consumption based on CPU and network utilization with an error of 3.3 percentage.








 

 
 
 
 





 
